On the nature of faint mid-infrared sources in M33

We investigate the nature of 24micron sources in M33 which have weak or no associated Halpha emission. Both bright evolved stars and embedded star forming regions are visible as compact infrared sources in the 8 and 24micron maps of M33 and contribute to the more diffuse and faint emission in these bands. Can we distinguish the two populations? We carry out deep CO J=2-1 and J=1-0 line searches at the location of compact mid-IR sources to unveil an ongoing star formation process. We use different assumptions to estimate cloud masses from pointed observations and analyze if SED and mid-IR colours can be used to discriminate between evolved stars and star forming regions. Molecular emission has been detected at the location of several sources at the level of 0.3 K km/s or higher in at least one of the CO rotational lines. Even though there are no giant molecular clouds beyond 4kpc in M33, our deep observations have revealed that clouds of smaller mass are very common. Sources which are known to be evolved variable stars show weaker or undetectable CO lines. Evolved stars occupy a well defined region of the IRAC color-color diagrams. Star forming regions are scattered throughout a larger area even though the bulk of the distribution has different IRAC colors than evolved variable stars. We estimate that about half of the 24 micron sources without an Halpha counterpart are genuine embedded star forming regions. Sources with faint but compact Halpha emission have an incomplete Initial Mass Function (IMF) at the high-mass end and are compatible with a population of young clusters with a stochastically sampled, universal IMF.

==> abstract <==
   We investigate the nature of  24\mi\ sources in M33 which have weak or no 
   associated  H$\alpha$ emission. Both bright evolved stars and embedded star forming
   regions are visible as compact infrared sources in the 8 and 24\mi\ {\it Spitzer} 
   maps of M33 and contribute to the more diffuse and faint emission in these bands.
   Can we distinguish the two populations ?
   We carry out deep CO J=2-1 and J=1-0 line searches at the location of 18 compact 
   mid-IR  sources and 2 optically selected ones
   to unveil an ongoing star formation process throughout the disk of M33. 
   We use different assumptions to estimate cloud masses from pointed
   observations. We also analyze if the spectral energy distribution  
   and mid-IR colours  can be used to discriminate between evolved stars and 
   star forming regions.  
   Molecular emission  has been detected at the location of 17 sources at the
   level of 0.3~K~km~s$^{-1}$ or higher in at least one of the CO rotational lines. Even though  
   there are no giant molecular clouds beyond 4~kpc in M33, our deep observations have revealed 
   that clouds of smaller mass are very common. Estimated molecular cloud masses range between 
   10$^4$ and 10$^5$~M$_\odot$, assuming likely values of the
   CO-to-H$_2$ conversion factor and virial equilibrium. Sources which are known to be 
   evolved variable stars show weaker or undetectable CO lines.  
   Evolved stars occupy a well defined  region of the IRAC color-color diagrams. Star forming regions
   are scattered throughout a larger area even though the bulk of the distribution has different 
   IRAC colors than evolved variable stars. We estimate that about half of the 24~\mi\ sources  
   without an H$\alpha$ counterpart are genuine embedded star forming regions.
   Sources with faint but compact H$\alpha$
   emission have an incomplete Initial Mass Function (IMF) at the high-mass end and 
   are compatible with a population
   of young clusters with a stochastically sampled, universal IMF.  
   
